Quicksort Is Optimal For Many Equal Keys

I prove that the average number of comparisons for median-of-$k$ Quicksort (with fat-pivot a.k.a. three-way partitioning) is asymptotically only a constant $\alpha_k$ times worse than the lower bound for sorting random multisets with $\Omega(n^\varepsilon)$ duplicates of each value (for any $\varepsilon>0$). The constant is $\alpha_k = \ln(2) / \bigl(H_{k+1}-H_{(k+1)/2} \bigr)$, which converges to 1 as $k\to\infty$, so Quicksort is asymptotically optimal for inputs with many duplicates. This resolves a conjecture by Sedgewick and Bentley (1999, 2002) and constitutes the first progress on the analysis of Quicksort with equal elements since Sedgewick's 1977 article.

==> equal-keys-fringe-balanced-trees.tex <==
% !TeX root = equal-keys-main





%\FloatBarrier

==> equal-keys-introduction.tex <==
\section{Introduction}

\todoin{write}
\begin{itemize}
\item
problem definition: sort $n$ numbers, \iid from universe of size $u$.
(think: $n\gg u\gg1$)
comparison model only.
\item
motivation: small universes common in practice (think: SQL GROUP BY);\\
	\iid assumption natural;\\
	corresponds to shuffled multiset,\\
	but problems are not exactly the same!
	
	$u$ can be small, but often not known up front;
	methods should adapt automatically.
	(\citet{SandeepGupta1999} call this idea \emph{distribution-sensitive})
\item
Sedgewick-Bentley: classic Quicksort optimal up to factor 2,
	conjecture: with sampling becomes optimal in leading term.
\item
comparison-based because universe is general
--> entropy lower bound
\item
Our Contributions:
	Sedgewick-Bentley conjecture confirmed (for large-entropy inputs),
	precise analysis of expected case for uniform universe distribution,
	same tricks help, and they help the same: multi-way partitioning and finite-size sampling
		yield same relative speedup as on random permutations
\item
NOT in this paper:
	other cost measures than ternary comparisons;
	actual multi-way partitioning methods;
\end{itemize}
\paragraph{The \iid Sorting Problem}

(discrete) \iid sorting: $n$ \iid elements from any (discrete) distribution


\paragraph{Fat-Pivot Quicksort}

~\\
\todoin{
	Add reference Quicksort as in \citet{Hennequin1991}:
	Based on lists, preserving order;
	sampled-out elements are the first in the subproblem.
}


\section{Related Work}

For the \textsl{multiset problem,} there are several known methods:
\todoin{write}
\begin{itemize}
\item
lower bounds: \citet{MunroRaman1991} give a simple argument via 2D vector sorting;
see ours below.
\item
simplest: collapse duplicates whenever they are first encountered.
\citet{MunroSpira1976} use that to describe Mergesort and Heapsort variants that are
optimal \wrt ternary comparisons up to lower order terms (linear in $n$).
The methods are not in-place though (the Heapsort uses a non-standard delete-max)
\item
SplaySort: insert into splay tree, marking/chaining equals is in $\Oh(\entropy(\vect q) n)$ 
(static optimality, Theorem~2 of \citet{SleatorTarjan1985}),
but the constant is at least $2$ (using semisplaying), and we need linear extra space.
\item
The first in-place method was the adapted Heapsort of \citet{MunroRaman1991};
it does not use the element-collapsing technique, but rather removes all duplicates from
the heap in one bulk extract-min operation.

\item
	Do all optimal algorithms have to be tweaked for multiset sorting explicitly?
	
	On the other hand;
	isn't fat-pivot partitioning tweaking as well?

\item
\citet{KatajainenPasanen1994} argue (indirectly) that a fat-pivot Quicksort
uses on average $2n\ln(n) - \sum_{v=1}^u x_v \ld(x_v) \wbin\pm \Oh(n)$ comparisons,
since ``Due to the three-way partitions, all redundant comparisons between a pivot and
elements equal to the pivot are avoided.''
Note however that this only shows that we use
\begin{align}
		\entropy(\vect x/n) n + (\tfrac2{\ld e}-1) n\ln n \bin\pm \Oh(n)
\end{align}
which is \emph{not} entropy-optimal.

\item
\notetoself{
	Counting cmps by outcome
	
	There are $n-u$ $=$-outcomes, because there are so many duplicates;
	and any more such outcomes would be redundant comparisons.
	The simple argument to separately count comparisons by outcome does not suffice to show
	optimality of Quicksort:
}

\item
\citet{SedgewickBentley2002} showed that Quicksort uses on average 
at most $\bigl(2\entropy(\vect x/n)+1\bigr)n$
comparisons to sort a random permutation of a multiset.
The technical results have long been known~\cite{Sedgewick1977a,AllenMunro1978}, 
they had just not been phrased in terms of multiset sorting.

\item
\citet{KatajainenPasanen1992a} demonstrate how to stably select medians in linear time
and use this to build a Quicksort-based sorting method that is entropy-optimal
up to a constant factor, even in the worst case. 
The average case will be roughly as the worst case.
Since the constant factor is at least $1+\alpha$ if $\alpha n$ comparisons
are need to select the median, this is not a competitive multiset sorting method.

\notetoself{
	Hashing can be used to map elements to $[1..u]$.
	We can then determine $u$ in a scan and classify elements using a binary search.
}

\item
Defense against other ways to solve this problem:
	radixsort/bucket sort: would have to learn/approximate distribution first,
		then essentially Quicksort;
		Devroye Theorem 3.1: $n$ in $[0,1]$ numbers with $n$ buckets is linear time 
			iff density square-integrable;

\end{itemize}

